MultiMUC: Multilingual Template Filling on MUC-4

We introduce MultiMUC, the first multilingual parallel corpus for template filling, comprising translations of the classic MUC-4 template filling benchmark into five languages: Arabic, Chinese, Farsi, Korean, and Russian. We obtain automatic translations from a strong multilingual machine translation system and manually project the original English annotations into each target language. For all languages, we also provide human translations for sentences in the dev and test splits that contain annotated template arguments. Finally, we present baselines on MultiMUC both with state-of-the-art template filling models and with ChatGPT.

==> appendices/word_alignment.tex <==
For word-to-word alignment using Awesome-align, we reused empirically-chosen hyperparameters from prior work for a similar task \cite{multicoref}: softmax normalization with probability thresholding of 0.001, 4 gradient accumulation steps, 1 training epoch with a learning rate of $2 \cdot 10^{-5}$, alignment layer of 16, and masked language modeling (``mlm''), translation language modeling (``tlm''), self-training objective (``so''), and parallel sentence identification (``psi'') training objectives. We additionally fine-tuned the resulting model, with the same hyperparameters, on 1200 English-Farsi, 2800 English-Chinese, and 2300 English-Arabic sentence pairs with gold word alignments, for 5 training epochs with a learning rate of $10^{-4}$ and ``so'' as the training objective.

